Intuitive Facial Animation Editing Based On A Generative RNN Framework

For the last decades, the concern of producing convincing facial animation has garnered great interest, that has only been accelerating with the recent explosion of 3D content in both entertainment and professional activities. The use of motion capture and retargeting has arguably become the dominant solution to address this demand. Yet, despite high level of quality and automation performance-based animation pipelines still require manual cleaning and editing to refine raw results, which is a time- and skill-demanding process. In this paper, we look to leverage machine learning to make facial animation editing faster and more accessible to non-experts. Inspired by recent image inpainting methods, we design a generative recurrent neural network that generates realistic motion into designated segments of an existing facial animation, optionally following user-provided guiding constraints. Our system handles different supervised or unsupervised editing scenarios such as motion filling during occlusions, expression corrections, semantic content modifications, and noise filtering. We demonstrate the usability of our system on several animation editing use cases.

==> generator.fig.tex <==

\begin{figure}[t]
  \centering
  \includegraphics[width=.30\textwidth]{../images/exports/generator.png}
  \caption{\
      \label{fig:generator}
    Architecture of the Generator
  }
  \Description{Architecture of the Generator }
\end{figure}


==> motion_adaptation_phnm.fig.tex <==

\begin{figure}[t]
  \centering
  \includegraphics[width=.4\textwidth]{../images/exports/motion_adaptation_phnm.png}
  \caption{\
      \label{fig:motion_adaptation_phnm}
      Our system modifies the jaw motion according to the input constraints such as adjusting the jaw opening to fit bilabial consonant constraints.
      Our system hallucinates micro-motions such as raising eyebrows to make the editing part more plausible.
  }
\end{figure}

